Search From the Start: Search-Native Pretraining for Language Models

Modern language models (LMs) are increasingly deployed with access to search tools at inference. Yet pretraining remains predominantly focused on predicting static text, with search capabilities typically introduced during post-training. We propose Search-Native Pretraining as a practical route to teach search capability during pretraining from ordinary text corpora. Specifically, we augment pretraining corpus at scale with web-search queries and retrieve web response using a local index. Training on this augmented corpus teaches models to generate search calls and incorporate retrieved evidence during language modeling. Across Wikipedia and DCLM-Edu corpora and 360M to 3.3B parameter scales, search-pretrained models ("QueryLM") show improved performance on knowledge-intensive tasks and higher steerability toward the retrieved evidence. Crucially, their advantage persists after supervised fine-tuning of both search-pretrained and conventionally pretrained models, indicating that the tested post-training procedures do not fully recover the capabilities developed during pretraining. Throughout our experiments, we find that a 1.4B QueryLM consistently beats or matches the performance of a FLOP-matched 3.3B baseline model across all knowledge intensive tasks. These results establish search-pretraining as a practical way to develop foundational search capabilities during pretraining. We release the training artifacts, including model checkpoints and data.

==> results_extra.tex <==
% ============================================================================
% Results moved out of the main Results section (2026-10-26, kept verbatim; NOT \input in main.tex).
% Uses the shared definitions in macros.tex.
% ============================================================================

% --- Wikipedia index ablation (Wikipedia Search-LLM 360M) ---
\begin{table}[t]
\centering
\caption{\textbf{\wikipedia{} index ablation, \wikipedia{} \model{} 360M} (accuracy, \%; identical model-written queries;
protocol of \Cref{tab:qa}). BM25 indexes the model's own 4.9M-document \wikipedia{} pretraining corpus; Tavily is
restricted to \texttt{en.wikipedia.org} (the setting used in \Cref{tab:qa}, shaded). The last column is the
fraction of retrieved contexts containing a gold answer (\triviaqa{} / NQ / \popqa{} / WebQs).}
\label{tab:wiki_backend}
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabular}{l c c c c c}
\toprule
\wikipedia{} index (context) & \triviaqa{} & NQ & \popqa{} & WebQs & Answer in context (\%) \\
\midrule
BM25, own corpus (raw, 1{,}200 chars)     & 19.3 & 3.3 & 6.3 & 4.0 & 66 / 25 / 28 / 25 \\
BM25, own corpus (compressed, 500 chars)  & 20.0 & 5.0 & 4.0 & 4.7 & 54 / 18 / 22 / 18 \\
\searchrow
Tavily, \wikipedia{} (compressed, 500 chars) & \textbf{27.3} & \textbf{8.7} & \textbf{6.7} & \textbf{6.3} & 60 / 36 / 30 / 28 \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{\wikipedia{} index.}
With the same model-written queries, the search engine over \wikipedia{} matters (\Cref{tab:wiki_backend}): Tavily
restricted to \wikipedia{} outperforms BM25 over the model's own pretraining corpus (27.3 vs.\ 20.0 on \triviaqa{}), and
accuracy follows the fraction of retrieved contexts that contain the answer.

% --- FreshQA by fact type / premise (DCLM-Edu 3.3B, base models) ---
\begin{table}[t]
\centering
\caption{\textbf{\freshqa{} \citep{vu2023freshllms} (21 April 2026 snapshot), \dclmedu{} 3.3B} (LLM-judged accuracy, \%;
500 test questions). Zero-shot; \model{} is forced to search with open-web search (queried in October 2026; gold answers
are as of the snapshot date). Superscript: gain over the compute-matched baseline.}
\label{tab:dclm_freshqa}
\small
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabular}{l l c c c c c}
\toprule
& & \multicolumn{3}{c}{Fact type} & \multicolumn{2}{c}{Premise} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-7}
Model & All & Never-changing & Slow-changing & Fast-changing & False & Valid \\
\midrule
\baselinehighlight   & 13.2 & 23.9 & 8.3 & 4.5 & \textbf{4.0} & 16.2 \\
\searchrow
\modelhighlight      & \textbf{28.4}\scoredelta{+15.2} & \textbf{42.6} & \textbf{24.4} & \textbf{13.6} & 3.2 & \textbf{36.7} \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Time-sensitive knowledge.}
On \freshqa{} (\Cref{tab:dclm_freshqa}), \model{} more than doubles the baseline's accuracy (28.4 vs.\ 13.2), with
gains on never- (+18.7), slow- (+16.1) and fast-changing facts (+9.1). Neither model handles false-premise questions
(3.2 vs.\ 4.0): both answer the presupposed question instead of rejecting it, and retrieval does not correct this.

% --- Previous discussion paragraphs (base models) ---
\Cref{tab:qa} shows our main results. \model{} answering with its own queries outperforms the compute-matched
baseline at every scale on every open-domain QA benchmark, and on average over all six tasks (+8.1 to +15.3). With \wikipedia{} pretraining at 360M, the open-domain average rises from 3.2 to 12.3,
comparable to \lmlm{} (13.8) with complementary strengths: \model{} is stronger on \triviaqa{} (27.3 vs.\ 15.3) and NQ, while
\lmlm{}'s knowledge base, built from \wikipedia{} entity facts, is stronger on \popqa{} (23.3 vs.\ 6.7). On knowledge multiple
choice, \model{} outperforms both the baseline (+9.5 \sciq{}, +2.9 \arceasy{}) and \lmlm{} (+4.0, +1.9).
With \dclmedu{} pretraining and open-web search, the open-domain average rises from 13--20\% to 35--40\%, and the 400M
\model{} (34.8) outperforms the 3.3B baseline (20.1). At the 360--400M scale, \model{} outperforms \colmlm{} with its full index
by 7.5 points on average (34.8 vs.\ 27.3) and on every benchmark, including long-tail \popqa{} (27.7 vs.\ 20.3). \colmlm{}
retrieves from a fixed index over its own training data, whereas \model{} queries an external search engine.
On multiple choice, \dclmedu{} models are much stronger than \wikipedia{} models (\sciq{} 74--83 vs.\ 38--47), since \dclmedu{}
contains educational science text; search still improves \sciq{} at every scale (+0.7 to +4.8 over the baseline), while on
\arceasy{}, which tests science reasoning more than fact lookup, gains are small at 400M and 1.4B and \model{} trails the
3.3B baseline (69.8 vs.\ 73.8).

\paragraph{Multi-hop QA.}
On the multi-hop datasets of the Search-R1 suite (\Cref{tab:dclm_searchr1}), \model{} outperforms the
compute-matched baseline on all four, by 5.6 points on average. The gain is largest on \hotpotqa{} (+11.6) and smaller on
the compositional 2Wiki (+3.6), \musique{} (+4.0) and \bamboogle{} (+3.2), consistent with pretraining on single-lookup
annotations: the model is not trained to chain dependent queries.

